Physics-based Digital Twins for Autonomous Thermal Food Processing: Efficient, Non-intrusive Reduced-order Modeling

One possible way of making thermal processing controllable is to gather real-time information on the product's current state. Often, sensory equipment cannot capture all relevant information easily or at all. Digital Twins close this gap with virtual probes in real-time simulations, synchronized with the process. This paper proposes a physics-based, data-driven Digital Twin framework for autonomous food processing. We suggest a lean Digital Twin concept that is executable at the device level, entailing minimal computational load, data storage, and sensor data requirements. This study focuses on a parsimonious experimental design for training non-intrusive reduced-order models (ROMs) of a thermal process. A correlation ($R=-0.76$) between a high standard deviation of the surface temperatures in the training data and a low root mean square error in ROM testing enables efficient selection of training data. The mean test root mean square error of the best ROM is less than 1 Kelvin (0.2 % mean average percentage error) on representative test sets. Simulation speed-ups of Sp $\approx$ 1.8E4 allow on-device model predictive control. The proposed Digital Twin framework is designed to be applicable within the industry. Typically, non-intrusive reduced-order modeling is required as soon as the modeling of the process is performed in software, where root-level access to the solver is not provided, such as commercial simulation software. The data-driven training of the reduced-order model is achieved with only one data set, as correlations are utilized to predict the training success a priori.

==> tiks/ROM-signal-tabs/MultiSineEqual15-Corr-a4-mod2.tex <==
\begin{table*}[htbp]
\footnotesize
\centering
\addtolength{\tabcolsep}{-2.1pt}
 \caption{Correlations between error measures (rows) and a priori and a posteriori excitation signal KPIs (columns) for APRBS 1-signal-ROMs (test set: MS15).} 
 \begin{tabular}{lrrrrrrrrrrrrrr} \toprule 
& $\overbar{T_i}$ & $\overbar{T_{\text{diff},i}}$ & $\overbar{T_{\text{diff},j}}$ & $\overbar{| T_{\text{diff},i} |}$ & $\overbar{T}_\text{oven}$ & STD($T_\text{oven}$) & Cr($T_\text{oven}$) & Cv($T_\text{oven}$) & Cv($T_\text{B}$) & Cv($T_\text{oven},T_\text{B}$)  & STD($T_\text{A}$)  & STD($T_\text{B}$) \\ 
\midrule 
RMSE   & 0.03            & 0.07                  & -0.05                 & -0.09                   & 0.04                    & 0.05               & 0.07              & 0.33              & 0.12             & -0.02                        & -0.15             & -0.18             \\
MAPE   & 0.12            & 0.02                  & -0.11                 & -0.02                   & 0.14                    & 0.04               & 0.03              & 0.34              & 0.13             & 0.06                         & -0.08             & -0.21             \\
MAX    & -0.21           & 0.12                  & 0.07                  & -0.21                   & -0.20                   & 0.08               & 0.12              & 0.23              & 0.02             & -0.16                        & -0.24             & -0.10             \\
MEDIAN & 0.07            & -0.56                 & -0.67                 & 0.29                    & 0.19                    & -0.03              & -0.07             & 0.10              & -0.40            & 0.13                         & 0.17              & -0.53             \\
IQR     & -0.12           & 0.20                  & 0.18                  & -0.30                   & -0.17                   & 0.13               & 0.17              & 0.21              & 0.16             & -0.27                        & -0.19             & 0.11              \\
$\text{R}^2$    & -0.17           & 0.34                  & 0.44                  & -0.15                   & -0.26                   & 0.07               & 0.10              & -0.27             & 0.12             & -0.15                        & -0.14             & 0.41               \\ 
\bottomrule 
 \label{tab:Corr-Show-a4-Eval-MultiSineEqual15} \end{tabular}\end{table*}

==> tiks/ROM-signal-tabs/sinAPRBSoldChi15-Corr-a4-mod.tex <==
\begin{table*}[htbp]
\footnotesize
\centering
\addtolength{\tabcolsep}{-2.1pt}
 \caption{Correlations between error measures (rows) and a priori and a posteriori excitation signal KPIs (columns) for APRBS 1-signal-ROMs (test set: sinAP15). } 
 \begin{tabular}{lrrrrrrrrrrrrrr} \toprule 
& $\overbar{T_i}$ & $\overbar{T_{\text{diff},i}}$ & $\overbar{T_{\text{diff},j}}$ & $\overbar{| T_{\text{diff},i} |}$ & $\overbar{T}_\text{oven}$ & STD($T_\text{oven}$) & Cr($T_\text{oven}$) & Cv($T_\text{oven}$) & Cv($T_\text{B}$) & Cv($T_\text{oven},T_\text{B}$)  & STD($T_\text{A}$)  & STD($T_\text{B}$) \\ 
\midrule 
RMSE   & 0.10            & -0.45                 & -0.68                 & 0.28                    & 0.22                    & -0.14              & -0.11             & 0.26              & -0.37            & 0.19                         & 0.01              & -0.72             \\
MAPE   & 0.16            & -0.43                 & -0.69                 & 0.34                    & 0.29                    & -0.13              & -0.12             & 0.26              & -0.32            & 0.26                         & 0.00              & -0.74             \\
MAX    & -0.04           & -0.52                 & -0.64                 & 0.15                    & 0.04                    & -0.17              & -0.07             & 0.24              & -0.47            & 0.01                         & 0.05              & -0.64             \\
MEDIAN & 0.18            & -0.43                 & -0.75                 & 0.48                    & 0.34                    & -0.08              & -0.13             & 0.19              & -0.35            & 0.39                         & -0.05             & -0.81             \\
IQR    & 0.04            & -0.25                 & -0.30                 & -0.08                   & 0.04                    & -0.12              & -0.01             & 0.27              & -0.17            & -0.17                        & 0.08              & -0.28             \\
$\text{R}^2$     & -0.15           & 0.42                  & 0.64                  & -0.28                   & -0.30                   & 0.14               & 0.12              & -0.26             & 0.27           & -0.22                        & -0.04             & 0.68             \\
\bottomrule 
 \label{tab:Corr-Show-a4-Eval-sinAPRBSoldChi15} \end{tabular}\end{table*}
